Characterizing Video Responses in Social Networks

Video sharing sites, such as YouTube, use video responses to enhance the social interactions among their users. The video response feature allows users to interact and converse through video, by creating a video sequence that begins with an opening video and followed by video responses from other users. Our characterization is over 3.4 million videos and 400,000 video responses collected from YouTube during a 7-day period. We first analyze the characteristics of the video responses, such as popularity, duration, and geography. We then examine the social networks that emerge from the video response interactions.

==> bibliography.tex <==
%\bibliographystyle{abbrv}


\begin{thebibliography}{99}

\bibitem{britney2007} A.  Zinman, J.  Donath  ``Is Britney Spears
Spam?'',  Fourth Conference on Email and Anti-Spam
CEAS 2007,  Mountain View, California.

\bibitem{liben2005}
D. Liben-Nowell, J. Novak, R. Kumar, P. Raghavan, and A. Tomkins.  Geographic Routing in social networks.  Proc. of National Academy of Sciences,
102(33):11623-11628, Aug. 2005.

\bibitem{lee2006}
S. Lee, P. Kim, and H. Jeong. Statistical Properties of Sampled Networks. Phys. Rev. E, 73:016102, 2006.

\bibitem{newman2003}
M. Newman and J. Park. Why Social Networks are Different from Other Types of Networks. Phys. Rev. E, 68:036122, 2003.

\bibitem{yong2007}
Y. Ahn, S. Han, H. Kwak, S. Moon, and H. Jeong.  Analysis of Topological Characteristics of Huge Online Social Networking Services, Proc. of  WWW
Conference, Banff, Canada, May, 2007.

\bibitem{eveline2006}  E. Velloso, V. Almeida, W.Meira, A. Bestavros, and S. Ji.
A hierarchical characterization of a live streaming media workload. IEEE/ACM Transactions on Networking,
14(1), 2006.

\bibitem{mendes2003}
S. Dorogovtsev and  J. Mendes.  Evolution of Networks: from Biological Nets to the Internet and WWW, Oxford University Press, 2003.

\bibitem{duarte2007}
F. Duarte, B. Mattos, A.  Bestavros, V.  Almeida, and J. Almeida.  Traffic Characteristics and Communication Patterns in Blogosphere, International
Conference on Weblogs and Social Media, Bouder, Colorado, March, 2007.

\bibitem{eveline2006}
E. Velloso, V. Almeida, W.  Meira, A.  Bestavros, and S. Ji.  A Hierarchical Characterization of a Live Streaming Media Workload, IEEE/ACM
Transactions on Networking, February, 2006.

\bibitem{newman2005}
M. Newman. Power laws, Pareto Distributions and Zipf's law, Contemporary Physics 46, 323-351, 2005.


\bibitem {stut2006}
D. Stutzbach, R. Rejaie, N.  Duffield, S. Sen, and W. Willinger, On Unbiased Sampling for Unstructured Peer-to-Peer Networks, Proc. of Internet
Measurement Conference, ACM SIGCOMM/Usenix, Rio de Janeiro, Brazil, 2006.


\bibitem{Cohen88}
J. Cohen, Statistical Power Analysis for the Behavioral Sciences, Hillsdale, NJ, 1988.


\bibitem{Newman2002b}
M. Newman.  Assortative Mixing in Networks.  Phys. Rev. Letters  89(20), 208701, 2002.

\bibitem{milgram}
S. Milgram.  The Small World Problem.  Psychology Today 2, 60-67, 1967.

\bibitem{wang}
D. Eppstein and J. Wang.  Approximation of Centrality, Journal of Graph Algorithms and Applications, 8(1), 39-45, 2004.

\bibitem{ebel}
H. Ebel, L. I. Mielsch, and S. Bornholdt.  Scale free topology of e-mail networks, Phys. Rev. E 66, 035103(R), 2002.

\bibitem{chau}
D. Chau, S. Pandit, S. Wang, and C. Faloutsos.  Parallel Crawling for Online Social Networks.  Proc. of  WWW Conference, Banff, Canada, May, 2007.

\bibitem{halvey}
M. Halvey and M. Keane.  Exploring Social Dynamics in Online Media Sharing.  Proc. of  WWW Conference, Banff, Canada, May, 2007.

\bibitem{latapy}
M. Latapy and C. Magnien.  Measuring Fundamental Properties of Real-World Complex Networks.  Available at arXiv.org:cs/0609115,2006

\bibitem{kumar}
R. Kumar, J. Novak and A. Tomkins. Structure and Evolution of Online Social Networks. Proc. of ACM SIGKDD Conference on Knowledge Discovery and Data
Mining, San Jose, CA, Aug, 2007.

\bibitem{shannon}  M.  Shannon, Shaking hands, kissing babies, and\...blogging?,
Communications of the ACM, vol. 50, no. 9, Sep. 2007, ACM Press  NY, USA.

\bibitem{mislove2007} A.  Mislove,  M. Marcon,  K. Gummadi, P. Druschel, B. Bhattacharjee, Proc. of ACM SIGCOMM/USENIX Measurement and Analysis of
Online Social Networks, Internet Measurement Conference 2007, Oct. 2007, San Diego, CA, USA

\bibitem{brin98} S. Brin and L. Page, The Anatomy of a Large-Scale Hypertextual Web Search Engine, Proc. of WWW Conference,  Brisbane, Australia,
May, 1998.

\bibitem{adamic07}  J. Zhang, M. Ackerman and L. Adamic, Expertise Networks in Online Communities: Structure and Algorithms, Proc. of WWW
Conference, Banff, Canada, May, 2007.

\bibitem{fonseca2005} R. Fonseca, V. Almeida and M. Crovella, Locality in a web of streams, Communications of the ACM, vol. 48, no. 1, 2005, ACM Press,
New York, USA.

\bibitem{fernando2007} F. Duarte, F. Benevenuto, V. Almeida, and J. Almeida. Geographical Characterization of YouTube: a Latin American View. Proc. of
LA-Web Conference, 2007, Santiago, Chile.

\bibitem{moon2007}
M. Cha, H. Kwak, P. Rodriguez, Y. Ahn, and S. Moon. I Tube, You Tube, Everybody Tubes: Analyzing the World's Largest User Generated Content Video
System.  Proc. of ACM SIGCOMM/USENIX Measurement and Analysis of Online Social Networks, Internet Measurement Conference 2007, Oct. 2007, San Diego,
CA, USA

\bibitem{facebook} S. Golder,  D. Wilkinson and B. Huberman, Rhythms of Social Interaction: Messaging
within a Massive Online Network, Proc. of the Int'l. Conf. on Communities and Technologies, 2007.


\bibitem{arlitt2007}
YouTube Traffic Characterization: A View From the Edge.  P. Gill, M. Arlitt, Z. Li and A. Mahanti. Proc. of ACM SIGCOMM/USENIX Internet Measurement
Conference 2007, Oct. 2007, San Diego, CA, USA


\bibitem{tomkins2003}
R. Kumar, J. Novak, P. Raghavan, and A. Tomkins. On the Bursty Evolution of Blogspace. In Proc. of the 12th
WWW Conference, Budapest, Hungary, May, 2003.

\bibitem{barabasi}  R. Albert, H. Jeong, and A.  Barabasi.  Diameter of the World Wide Web,  Nature 401, 130-131 (1999).

\bibitem{kleinberg199} J. Kleinberg, `Hubs, Authorities, and Communities,
ACM Comput. Surv., vol 31,  no 4es, 1999, ACM, New York, NY, USA

\bibitem{adamic07b} N. Ali-Hasan and L. Adamic. Expressing Social Relationships on the Blog through Links and Comments, ICWSM2007, March 2007, Boulder, CO.
\bibitem{molina2007} P. Heymann, G. Koutrika, H. Garcia-Molina, "Fighting Spam on Social Web Sites: A Survey of Approaches and Future Challenges," IEEE Internet Computing, vol. 11, no. 6, Nov/Dec, 2007.

\end{thebibliography}
















==> userbehavior.tex <==


\section{Spam, Promotion, and Anti-Social Behavior }
\label{sec:behavior}

Different forms of unsolicited communication are taking a toll on users of social networking services~\cite{britney07}. Unsolicited communication opens a large gray area, where videos could be considered spam, promotion or unsolicited advertising.  Spam and promotion take different forms in online social video networks. The simplest form of spam occurs when users submit a video with a long list of misleading tags to describe its content. The purpose is to fool video searching mechanisms. Frequently, spam and promotion appear in textual comments and video responses. In most of the cases, spammers and users looking for promotion attempt to boost the ranking of their videos to make them highly visible in the social network ranks.   Due to its intrinsic nature, video response appears to be an attractive feature to users aiming at distributing different types of spam and promotion, including self-promotions and product advertising. Unlike textual responses or comments, one has to start the streaming and view it to realize the specific video is some form of spam or promotion.  A simple example illustrates how anti-social behavior, such as distribution of spam, self-promotion and unexpected advertising, could  be identified by examining patterns of user behavior in a social networking service.  Figure~\ref{fig:resp_userrank} shows that the distribution of the number of video responses posted by  responsive users follows a power law. Experimental data have been used in the literature to show the behavior of many real-world systems can be modeled by a power law distribution. We notice from the figure that three points do not fit the expected power law. They represent users that have posted a very large number of video responses. By identifying these users in our dataset, we realized they share common characteristics: i) they are users that post video responses to either their own videos or to other specific videos to boost their rankings in order to increase their visibility and ii) they are users that make use of video responses as a marketing opportunity in the social networking environment, spreading video-based information to influence others or to advertise commercial products and services.  

Interestingly, it seems that mechanisms and algorithms to fight the distribution of spam and other forms of polluted content in social networking should primarily focus on the user rather than the message, i.e., the video. In this we focus on the use of metrics that help to understand different types of users that participate in video-based interactions in social networks. 
 

\subsection{Characterizing  User Behavior}

The previous example shows how patterns of video-based interactions might correlate with a user's behavior in social networking sites. Next we analyze characteristics of user behavior that could be used to design algorithms to fight spam and information pollution in online social video networks.  
Simple features can be used as a first cut in the identification of anti-social behavior. For example, users who upload much more video responses that receive response to
their videos, as shown by the In-Out degree ratio in Figure~\ref{fig:inoutratio}, are potential candidates for an in-depth analysis of their behavior. This section
proposes a simple metric that represent the way users participate in a sequence of responses to video $i$. We define the inter-reference distance (IRD) on the sequence of
users that upload video responses to video $i$ as the total number of responses that appear between two video responses from the same user. Previous studies on
spam characterization refer to the importance of temporal issues of the distribution. For example, whereas traditional e-mail traffic is concentrated on diurnal periods,
the arrival rate of spam e-mails is roughly stable over time.~\cite{lhg2007}. With IRD, we want to assess temporal patterns of the users' participation in a sequence of
video responses. Figure~\ref{fig:irdvscount} plots for each responsive user the average IRD and the average response per video. A user that uploads many responses per
video, one after the other, like a mechanical process, might be a candidate for further investigation.   Thus, the combination of a large number of responses per video
and small IRD suggests the user has some type of anti-social behavior.  We conducted an initial investigation to verify if the combination of two metrics (i.e., IRD and
average responses per video) could accurately be used to identify users with anti-social behavior. Our experiment focus  on users that are located on the rightmost part
of Figure~\ref{fig:irdvscount}. In the dataset, a total of 298 users have average IRD less than 3 and average number of responses per video greater than 10. A group of  5
volunteers in our laboratory randomly selected 95 users, which represent the dataset with a confidence interval of 90\% and an error of 7\%.  Our volunteers then viewed the
users' video responses and classified responsive users into two categories, according to the content of their video: social or anti-social user.  If at least one video response is considered spam, promotion or advertising,
the responsive user is labeled as anti-social. It should be observed that the human classification process carries a certain degree of subjectivity. The volunteers viewed
a large percentage of the videos of each responsive user. A total of the 80\% users that meet the specified requirements were classified as anti-social user, suggesting
that the proposed metrics could be a starting point to develop heuristics to combat video spam in social networks.
 
\begin{figure}[Hhtb]
\centering
\includegraphics[width=.3\textwidth]{fig/interreferencedistance_mean_per_count_user_col_3.eps}
\caption{Inter Reference Distance vs Average Responses per Video.
}
\label{fig:irdvscount}
\end{figure}


\subsection{User Rank}

The next step is to use the structure of the social network for detecting anti-social patterns. Instead of using node local properties such as degree distribution to represent the importance of a user in the network, we use the Pagerank~\cite{brin98} algorithm, on the video response user graph, to determine ``user rank''. 
Basically, in the PageRank algorithm, a user has a high rank if the page has many incoming links and when a user has a few links coming from highly ranked users. We call the scores computed by the algorithm as UserRank, which could be used as an indicator of the importance of users in terms of their participation in video interactions. The calculated correlation between UserRank and in-degree is 0.13, suggesting that the relationship between the two metrics is weak.  Figure~\ref{fig:pagerank} shows  the  UserRank distribution for  the user network  using a complementary  cumulative distribution function (i.e., $1-CDF$) plot. The figure shows that there is  strong correlation between UserRank and total number of views of the user's videos, suggesting the algorithm captures the importance of users in terms number of views.  We randomly selected a few users have either high rank or low rank.  We verified their profiles and their video response. Users with high rank are among the most viewed and most subscribed users. Most of them are directors (i.e, a director accounts have special advanced options in YouTube). Low rank users have small number of views and some of them exhibit some of the characteristics already discussed in this section, namely,
they post video responses to many videos but receive no video responses from the video community.     





\begin{figure}[Hhtb]
\centering
\includegraphics[width=.3\textwidth]{fig/graph/ownersvideoresponse.direct.number.sort.pagerank.normalised.ccdf.eps}
\includegraphics[width=.3\textwidth]{fig/graph/ownersvideoresponse.direct.number.sort.pagerank.nviews.eps}
\caption{UserRank Distribution (top) and UserRank Correlated with Number of Views (bottom).
%he Other Figure correlates the total views of the videos of each user and its UserRank
}
\label{fig:pagerank}
\end{figure}






==> videolevel.tex <==
\vspace{-0.1cm}
\section{Video-Based Interactions}

Our characterization of user interactions at the video level consists of examining the sequence
of video responses following a YouTube video. For each responded video $V_i$, let $n_i$ denote
the number of video responses, and denote the sequence of responses as
$\{VR_{i,1}; VR_{i,2}; ...; VR_{i,j}; ... ; VR_{i,n_i} \}$,
where $VR_{i,j}$ is the $j^{th}$ video response.

A user may add multiple video responses in sequence to the same video. We define a
sequence of responses $S_{i,k}$ as a series of {\em consecutive} responses from the same user to
video $V_i$. Thus, the ordered list of video responses to video $i$ can be also expressed as
$\{S_{i,1}; S_{i,2}; ... S_{i,s_i} \}$, $1 \le s_i \le n_i$,
where $S_{i,k}$ is the sequence $\{ VR_{i,j}; VR_{i,j+1} ... \}$ of {\it consecutive} responses from
user $U_{i,k}$.
Note that the same user may post multiple (non-consecutive) sequences of responses  to the same video $V_i$, i.e., we may  have $U_{i,k} = U_{i,j}$ for $k$ $\not\in$ [j-1,j+1].

In the following example, video $V_i$ received 7 video responses grouped into 4 sequences, posted by 3
different users ($U_{1}$, $U_{2}$ and $U_{3}$):


$$
V_i; \overbrace{\underbrace{VR_{i,1}, VR_{i,2}}_{U_1}}^{S_{i,1}},\overbrace{\underbrace{VR_{i,3}}_{U_2}}^{S_{i,2}}, \overbrace{\underbrace{VR_{i,4}, VR_{i,5},VR_{i,6}}_{U_1}}^{S_{i,3}}, \overbrace{\underbrace{VR_{i,7}}_{U_3}}^{S_{i,4}}
$$

Our characterization focuses on a simple metric,
defined as the ratio U-S of the {\em Number of Unique Responsive Users} to the
{\it Number of Sequences of Responses}.
In the above example, this ratio is 0.75.
A video-based interaction with a ratio U/S close to
0 indicates an asynchronous video dialogue between a relatively small number of highly active users,
who keep the discussion alive with multiple (not necessarily consecutive) responses to each other.
This type of interaction is akin to the exchanges and debates in a
parlor or public forum, in which the communication underscores a many-to-many dialogue between participants.
At the other extreme, when the ratio  approaches one, there may be two types of interaction.
One type occurs when the number of unique responsive users  equals the number of sequences of responses,
resembling a register, petition or guest-book,
for which the communication is many-to-one, and the purpose of a video response is to record a comment
(or support a petition, etc.). The other type has just one user posting a single sequence.

Figure~\ref{fig:pvi} (right) shows the ratio U/S versus the number of
sequences of responses for each responded video in our data set.
Different types of interactions can be seen across all responded videos,
characterized by a wide range of U-S values. However, only a relatively small number of
videos triggered lively interactions, with each responsive user adding on average at least 3 sequences of responses.
In fact,  the vast majority of the responded videos (99\%) triggered
interactions with only  one sequence of responses per responsive user  (i.e., ratio equal to 1).
In fact, Figure \ref{fig:pvi} (right) shows these interactions
occur among groups of responsive users of  varying sizes (i.e., number of sequences).





